Asymptotically Optimal Repair of Reed-Solomon Codes with Small Sub-Packetization under Rack-Aware Model

This paper presents a comprehensive study on the asymptotically optimal repair of Reed-Solomon (RS) codes with small sub-packetization, specifically tailored for rack-aware distributed storage systems. Through the utilization of multi-base expansion, we introduce a novel approach that leverages monomials to construct linear repair schemes for RS codes. Our repair schemes which adapt to all admissible parameters achieve asymptotically optimal repair bandwidth while significantly reducing the sub-packetization compared with existing schemes. Furthermore, our approach is capable of repairing RS codes with asymptotically optimal repair bandwidth under the homogeneous storage model, achieving smaller sub-packetization than existing methods.

==> IEEE-RPA-results.tex <==
\bibitem{facebook} S. Muralidhar, W. Lloyd, S. Roy, C. Hill, E. Lin, W. Liu, et al., ``f4: Facebook's warm BLOB storage system," in proc. 11th USENIX Symposium on Operating Systems Design and Implementation (OSDI),2014, pp. 383-398.

\bibitem{google} Colossus: Successor to the google file system. \url{http://www.systutorials.com/3202/colossus-successor-to-google-file-system-gfs/}.

\bibitem{baidu} C. Lai, S. Jiang, L. Yang, S. Lin, G. Sun, Z. Hou, et al., ``Atlas: Baidu's key-value storage system for cloud data," in proc. 31st Symposium on Mass Storage Systems and Technologies (MSST). IEEE, 2015, pp. 1-14. DOI: 10.1109/MSST.2015.7208288

\bibitem{mic} C. Huang, H. Simitci, Y. Xu, A. Ogus, B. Calder, P. Gopalan, et al., `` Erasure coding in windows azure storage," in proc. 2012 USENIX Annual Technical Conference (USENIX ATC 12). 2012, pp. 15-26.

\bibitem{Gu} V. Guruswami and M. Wootters, ``Repairing Reed-Solomon codes,” IEEE Trans. Inf. Theory, vol. 63, no. 9, pp.~5684–5698, Sep. 2017.

\bibitem{Dau1} H. Dau and O. Milenkovic, ``Optimal repair schemes for some families of full-length Reed-Solomon codes,” in Proc. IEEE Int. Symp. Inf.Theory (ISIT), Jun. 2017, pp. 346–350. DOI: 10.1109/ISIT.2017.8006547

\bibitem{Ye1} M. Ye and A. Barg, ``Explicit constructions of MDS array codes and RS codes with optimal repair bandwidth," in Proc. IEEE Int. Symp. Inf. Theory (ISIT), Jul. 2016, pp. 1202-1206. DOI: 10.1109/ISIT.2016.7541489

\bibitem{Ye2} I. Tamo, M. Ye, and A. Barg, “Optimal repair of Reed-Solomon codes: Achieving the cut-set bound,” in Proc. 58th Annual IEEE Symp. Founda tions Computer Sci. (FOCS), Oct. 2017, pp. 216-227. DOI: 10.1109/FOCS.2017.28

\bibitem{Li} W. Li, Z. Wang, and H. Jafarkhani, ``On the sub-packetization size and the repair bandwidth of Reed-Solomon codes,'' IEEE Trans. Inf. Theory, vol. 65, no. 9, pp.~5484--5502, Sep. 2019. DOI: 10.1109/TIT.2019.2917425

\bibitem{Vardy} A. Chowdhury and A. Vardy, ``Improved schemes for asymptotically optimal repair of MDS codes,'' IEEE Trans. Inf. Theory, vol. 67, no. 8, pp.~5051--5068, Aug. 2021. DOI: 10.1109/TIT.2021.3071447

\bibitem{Hu1} Y. Hu, P. P. Lee, and X. Zhang, ``Double regenerating codes for hierarchical data centers,” in Proc. IEEE Int. Symp. Inf. Theory (ISIT), Jul. 2016, pp. 245–249. DOI: 10.1109/ISIT.2016.7541298

\bibitem{Hou1} H. Hou, P. P. Lee, K. W. Shum, and Y. Hu, ``Rack-aware regenerating codes for data centers,” IEEE Trans. Inf. Theory, vol. 65, no. 8, pp.~4730–4745, Aug. 2019. DOI: 10.1109/TIT.2019.2902835

\bibitem{Chen1} Z. Chen and A. Barg, ``Explicit Constructions of MSR Codes for Clustered Distributed Storage: The Rack-Aware Storage Model,'' IEEE Trans. Inf. Theory, vol. 66, no. 2, pp.~886--899, Feb. 2020. DOI: 10.1109/TIT.2019.2941744

\bibitem{Jin} L. Jin, G. Luo, and C. Xing, ``Optimal repairing schemes for Reed- Solomon codes with alphabet sizes linear in lengths under the rack-aware model,” arXiv:, Nov. 2019.

\bibitem{wang2023} J. Wang and Z. Chen, ``Low-access repair of Reed-Solomon codes in rack-aware storage" in Proc. IEEE Int. Symp. Inf. Theory (ISIT), Jun. 2023, pp. 1142-1147.


